Une liste de probl\`emes

This is a structured compilation of some of my favourite open problems.

==> arxivlistepb.tex <==
arXiv


Une liste de probl\`emes

A paraitre dans

A paraître dans Mathematics Going Forward, Collected Mathematical Brushstrokes,
Springer LNM 2313, 2023

https://link.springer.com/book/9783031122453

Summary

This is a structured  compilation of some of my favourite open problems. It will appear in
the book Mathematics Going Forward, Collected Mathematical Brushstrokes, Springer, 2022.


AMS codes

14-01 14-02 14D10 14E08 14G12
